Exact and Approximate Methods for Proving Unrealizability of Syntax-Guided Synthesis Problems

We consider the problem of automatically establishing that a given syntax-guided-synthesis (SyGuS) problem is unrealizable (i.e., has no solution). We formulate the problem of proving that a SyGuS problem is unrealizable over a finite set of examples as one of solving a set of equations: the solution yields an overapproximation of the set of possible outputs that any term in the search space can produce on the given examples. If none of the possible outputs agrees with all of the examples, our technique has proven that the given SyGuS problem is unrealizable. We then present an algorithm for exactly solving the set of equations that result from SyGuS problems over linear integer arithmetic (LIA) and LIA with conditionals (CLIA), thereby showing that LIA and CLIA SyGuS problems over finitely many examples are decidable. We implement the proposed technique and algorithms in a tool called Nay. Nay can prove unrealizability for 70/132 existing SyGuS benchmarks, with running times comparable to those of the state-of-the-art tool Nope. Moreover, Nay can solve 11 benchmarks that Nope cannot solve.

==> approx.tex <==
\section{Approximation of Conditional Tree grammars on Examples}

\heping{1. Substitute variables $v$ with some approximation $\alpha(v)$.
	2. interpret productions as  expression over the approximation
	3. Solve the expression to find approximation of the grammar
	4. how to deal with ITE}

\section{A decidable fragment of SyGuS Problems}
\heping{1.}

==> conclusion.tex <==
% -*- TeX-master: t; TeX-PDF-mode: t -*-

\section{Conclusion}
\label{Se:Conclusion}

We presented a technique for  automatically establishing that a
given syntax-guided-synthesis (\sygus) problem is
unrealizable (i.e., it has no solution). 
Our technique encodes the problem of proving that a \sygus problem is unrealizable over a finite set of examples
into that of solving a set equations over sets of values---i.e., an abstract domain. 
The  solution to the set of
equations gives us an overapproximation of the set of possible outputs that any term in the problem search space can produce on the given input examples. If none of the possible outputs meets the specification, 
the \sygus problem is unrealizble.
This technique connects the problem of proving unrealizability to that of solving equations over abstract domains.
Because this latter problem has recently received great interest due to its connection to program analysis,
our technique directly inherits many of the new developed results in solving equations over abstract domains.
For example, we have presented techniques for exactly solving equations for \sygus problems over the theories of 
linear integer arithmetic (LIA) and  linear integer arithmetic with conditionals (CLIA).
Our prototype implementation, \name, could prove unrealizability for 5
new problems that eluded existing techniques.
%\loris{open problems: what other domains, what does this tell us about verification, what about the other way around?}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> newton.tex <==
\section{Newton's Method for Conditional Communicative Grammars}
We define three functions $\slv:N_{\texttt{int}}\to2^{\mathbb{Z}^{|E|}}$, $\slt:N_{\texttt{int}}\to2^{\mathbb{Z}^{\Sigma^{(0)}+1}}$ and $\bv:N_{\texttt{bool}}\to2^{\mathbb{B}^{|E|}}$. 

==> otherDomain.tex <==
% -*- TeX-master: t; TeX-PDF-mode: t -*-

\section{Incomplete Techniques for Grammars Beyond LIA and CLIA}
\label{Se:other-domains}


In this section, we present two sound but incomplete techniques that let us to use
GFA to handle  grammars beyond the ones
discussed in \sectref{ProvingUnrealizabilityOfSyGuSProblemsInLIA} and \sectref{SolvingSyGuSProblemsInCLIA}.
First, we show how grammar flow analysis can easily accommodate predicate abstraction---i.e., any abstract domain consisting of finitely many predicates (\sectref{predicate-abstraction}).
Second, we show how equations over arbitrary decidable theories can be encoded as
constrained horn clauses that can be solved using sound but incomplete solvers such as Z3~\cite{z3}.


\subsection{Predicate Abstraction}
\label{Se:predicate-abstraction}

In predicate abstraction, the abstract semantics of a term is given
via a finite set of predicates $\paset=\{\varphi_1,\ldots,\varphi_n\}$.
For the convenience of use in grammar flow analysis, we introduce the
following, slightly non-standard formalization of predicate abstraction:
we assume that the predicates in $\paset$ are disjoint, and their union
is equivalent to true.
Concretely, for each expression $e$, the abstract semantics is given by 
a set $\semgamma{e}_E\subseteq \paset$ denoting that
the expression $e$, when evaluated on the examples $E$, produces an output $o$
that satisfies the  predicate:
$\bigvee_{\varphi\in\semgamma{e}_E} \varphi(o)$. \john{Should it be $\bigwedge$ instead $\bigvee$?}

%Our technique for proving unrealizability via grammar-flow analysis can be easily applied to any predicate-abstraction-based
%abstract domain.
Because the set $\paset$ is finite, it is easy to always define a (potentially imprecise) abstract semantics 
for any symbol with any concrete semantics and
define the combine of two elements $\Phi_1$ and $\Phi_2$ in the abstract domain $2^\paset$
as $\Phi_1\oplus \Phi_2=\Phi_1\cup \Phi_2$.
Because $\paset$ is finite, the set of equations obtained via GFA can always be solved
using an iterative algorithm that terminates in at most $2^{|\paset|}$ iterations as done in \sectref{booleanonly}.
%We already applied this idea in \sectref{booleanonly}, where we used sets of Booleans as an (exact) 
%predicate-abstraction domain.
%In fact, any finite domain of values $V$ of size $n$ can be exactly (though inefficiently) modeled using a predicate abstraction domain 
%$\paset_V$ of size $2^n$.

\begin{example}
\label{Ex:parity}
Consider the \sygus problem $(f(x)=1,G_p)$ where the grammar $G_p$
is the following:
\[
\begin{array}{c}
\Start	::= \textrm{Times2}(\SOne) \qquad\qquad
\SOne 	::=  \textrm{Plus1}(\SOne) \mid \textrm{Num}(1) \\
\end{array}
\]
where 
$\sem{\textrm{Plus1}(e)}_E=\sem{e}_E+1$
and $\sem{\textrm{Times2}(e)}_E=\sem{e}_E*2$.
Suppose we are given an example set $E=\B{i_0}$. 
An example of a predicate-abstraction-based domain for
describing the semantics $\semgamma{e}_E$ of an expression 
is the set of predicates
$\paset_p=\{odd(x), even(x)\}$ that denote whether the output of an expression on
input $i_0$ is  odd or even, respectively.

%Because of the new symbols, the techniques presented in \sectref{ProvingUnrealizabilityOfSyGuSProblemsInLIA} and \sectref{SolvingSyGuSProblemsInCLIA} cannot directly help us prove unrealizability for this \sygus problem.
We can use the predicate set $\paset_p$ to define the abstract semantics:
$\semgamma{\textrm{Plus1}}_E(P)=\paset_p\setminus \Phi$ 
\iffull(i.e., adding 1 to a number changes its parity)\fi
and $\semgamma{\textrm{Times2}}_E(\Phi)=\{even(x)\}$.
Solving the equations resulting from the grammar $G_{par}$ will yield the following solution:
$n(\Start)=\{even(x)\}$ and $n(S1)=\paset_p$, with which we can prove that the problem is unrealizable because $o=1 \wedge even(o)$ is unsatisfiable.
\qed
\end{example}

Predicate abstraction is a very versatile technique, but it is imprecise---i.e., it cannot exactly capture the set of 
possible outputs produced by the expressions in the grammar. 
\iffull
For example, consider the following grammar  $G_{3x}$ generating only LIA terms:
\[
\begin{array}{rcl}
  \Start & ::= & \textrm{Plus}(\Start, \Start) \mid \textrm{Num}({3})
\end{array}
\]
When using the predicate abstraction domain $\paset_p$ from Example~\ref{Ex:parity},
solving the set of equations resulting from the grammars will result in the very imprecise 
value
$n(\Start)=\paset_p$.
On the other hand, the technique presented in \sectref{ProvingUnrealizabilityOfSyGuSProblemsInLIA}
will produce an exact value for $n(\Start)$.
\fi
Moreover, it is hard to choose the set $\paset$ and in common uses of predicate abstractions,
this set is continuously refined through automated techniques. 



	
	\subsection{Grammar Flow Analysis using Horn Clauses}
\label{Se:HornClauses}	
	
	In this section, we define the \heping{(complete combine?)} semilattice $(\fpred,\vee)$ and then show that how to prove unrealizability of \sygus problems with \LIA grammars. 
	
	The domain $\fpred$ contains all first-order predicate in \LIA. The combine $\vee$ is the logical disjunction of predicates. The order for two predicates $\phi_1,\phi_2$, $\phi_1\le\phi2$ iff for all models $\vec{v}$ we have $\phi_1(\vec{v})\implies\phi_2(\vec{v})$.
	
	For the semi-lattice of first order predicates, we rewrite \eqref{GFA} as
	\begin{eqnarray}
		n_\calG(X_0) \ge \bigvee_{X_0 \to g(X_1, \ldots, X_k) \in \delta} \semgamma{g}_P(n_\calG(X_1), \ldots, n_\calG(X_k)),
	\end{eqnarray}
	where the interpretation to the operators are defined as follows:

			\begin{eqnarray}
			\semgamma{\textrm{Plus}}_P(\phi_1,\phi_2) & = & \vec{v}=\vec{v_1}+\vec{v_2}\wedge\phi_1(\vec{v_1})\wedge\phi_2(\vec{v_2}) \\
			\semgamma{\textrm{Num}(c)}_P         & = & \vec{v}=\vec{c}\\
			\semgamma{\textrm{Var}(x)}_P & = & \vec{v}=\mu_E(x) \\
			\semgamma{\textrm{NegVar}(x)}_P & = & \vec{v}= -\mu_E(x)
			\end{eqnarray}

Note that the equations now are in Horn clause format. 

\begin{example}
	
\end{example}


